On the Role of Information Structure in Reinforcement Learning for Partially-Observable Sequential Teams and Games

In a sequential decision-making problem, the information structure is the description of how events in the system occurring at different points in time affect each other. Classical models of reinforcement learning (e.g., MDPs, POMDPs) assume a simple and highly regular information structure, while more general models like predictive state representations do not explicitly model the information structure. By contrast, real-world sequential decision-making problems typically involve a complex and time-varying interdependence of system variables, requiring a rich and flexible representation of information structure. In this paper, we formalize a novel reinforcement learning model which explicitly represents the information structure. We then use this model to carry out an information-structural analysis of the statistical hardness of general sequential decision-making problems, obtaining a characterization via a graph-theoretic quantity of the DAG representation of the information structure. We prove an upper bound on the sample complexity of learning a general sequential decision-making problem in terms of its information structure by exhibiting an algorithm achieving the upper bound. This recovers known tractability results and gives a novel perspective on reinforcement learning in general sequential decision-making problems, providing a systematic way of identifying new tractable classes of problems.

==> proof/ucb/estimation_guarantee.tex <==
\subsection{Estimation guarantee}\label{ssec:proof_est_guarantee}
The following result states that the estimated model is accurate on the past exploration policies and dataset of collected trajectories. This holds for both the conditional probabilities of futures given past trajectories in the dataset as well as over full trajectories. The result follows from~\Cref{prop:mle_E_omega,prop:mle_E_pi,prop:mle_E_min} in the MLE analysis of the previous section.
\begin{lemma}\label{lemma:estimation_guarantee}
    Let $\beta = 31 \log \frac{K \abs{\bar{\Theta}_\varepsilon}}{\delta}$, and suppose $\varepsilon \leq \frac{\delta}{K^2 H^2 \prod_{h}\abs{\bbX_{h}}}$, where $\bar{\Theta}_{\varepsilon}$ is the optimistic $\varepsilon$-net in~\Cref{prop:optimistic_eps_net}. Then, under event $\calE$, the following holds,
    \begin{align*}
        &\sum_h \sum_{(\tau_h, \pi) \in \calD_h^k} \tvsq{\probb{\hat{\theta}^k}{\pi}(\omega_h | \tau_h), \probb{\theta^*}{\pi}(\omega_h | \tau_h)} \leq 7 \beta, \text{and}\\
        &\sum_{\pi \in \calD^k} \hellingersq{\probb{\hat{\theta}^k}{\pi}(\tau_H), \probb{\theta^*}{\pi}(\tau_H)} \leq 7 \beta, \\
    \end{align*}
\end{lemma}
\begin{proof}
    Lemma 1 of~\cite{huangProvablyEfficientUCBtype2023}.
\end{proof}

% used to be its own section, but merged with general MLE results

==> seq_teams_psr_rank.tex <==
\section{Bounding the rank of system dynamics via information structure and \texorpdfstring{$d$}{d}-separation}\label{sec:seq_teams_psr_rank}

% \subsection{Motivation: PSR rank of POMDPs}

In this section, we will show that the information structure of a sequential team can be used to obtain a bound on the rank of the system dynamics matrices $\bm{D}_h$ (which coincides with the PSR rank). The main tool in doing so is the DAG representation $\calG$ of the information structure $\set{\calI_t, t \in [T]}$. To motivate this, we recall a classic result on PSRs (see e.g. Theorem 1 of~\cite{littmanPredictiveRepresentationsState}).

\begin{example*}[POMDPs have PSR rank bounded by $\abs{\bbS}$]
    Consider a POMDP with states $s_t \in \bbS$, observations $o_t \in \bbO$, and actions $a_t \in \bbA$. The system dynamics are given by $\prob{s_{t+1}, o_{t+1} \given s_{1:t}, a_{1:t}, o_{1:t}} = \prob{s_{t+1} \given s_t, a_t} \prob{o_{t+1} \given s_{t+1}}$. We will derive a bound on the PSR rank of this partially observable system. For each history $\tau_t = \paren{o_1, a_1, \ldots, o_t, a_t}$ and a future $\omega_t = \paren{o_{t+1}, a_{t+1}, \ldots o_T, a_T}$, we have,
    \begin{equation*}
            \bm{D}_{\tau_t, \omega_t} = \prob{\tau_{t}^o, \omega_t^o \given \mathrm{do}(\tau_t^a, \omega_t^a)} = \sum_{s_{t+1} \in \bbS} \prob{\omega_{t} \given s_{t+1}} \prob{s_{t+1} \given \tau_t} \prob{\tau_t^o \given \tau_t^a}.
    \end{equation*}

    Hence, defining $\bm{D}_{t, 1} := \bra{\prob{\omega_{t} \given s_{t+1}}}_{\omega_{t}, s_{t+1}}$ and $\bm{D}_{t,2} := \bra{\prob{s_{t+1} \given \tau_t} \prob{\tau_t^o \given \tau_t^a}}_{s_{t+1}, \tau_t}$, we have that $\bm{D}_t = \bm{D}_{t,1} \bm{D}_{t,2}$. Thus, $\mathrm{rank}(\bm{D}_t) \leq \abs{\bbS}$ for all $t$. Hence, the rank of the observable dynamics of a POMDP is bounded by the number of states.

    \hfill $\square$
\end{example*}

In the above, the existence of a latent state implied a simplification of the dynamics and a bound on the rank. We will use the same intuitive idea to bound the rank of the observable dynamics of partially-observable sequential teams via their information structure.

\begin{definition}\label{def:G_dagger}
    $\calG^\dagger$ is the DAG obtained from $\calG$ by removing all edges directed towards actions. That is, it consists of the edges $\calE^\dagger \coloneqq \calE \setminus \set{(x, a): x \in \calN, a \in \calA}$.
\end{definition}

Removing the incoming edges in the action variables in $\calG^\dagger$ corresponds to the $\mathrm{do}$ operation in the definition of the system dynamics matrix in~\Cref{eq:seq_team_dynamics_mat}.

\begin{definition}[Information-structural state]\label{def:I_dagger}
    For each $h \in [H]$, let $\calI_h^\dagger \subset [t(h)]$ be the minimal set of past variables (observed or unobserved) which $d$-separates the past observations $\paren{X_{t(1)}, \ldots, X_{t(h)}}$ from the future observations $\paren{X_{t(h+1)}, \ldots, X_{t(H)}}$ in the DAG $\calG^\dagger$. Define $\bbI_h^\dagger := \prod_{s \in \calI_h^\dagger} \bbX_s$ as the joint space of those variables.
\end{definition}

The notation $\calI_h^\dagger$ is chosen to emphasize that this set depends on the information structure, $\calI = \set{\calI_t, t \in \calN}$, and that it somehow simplifies or ``inverts'' the dynamics. Note also that $\calG^\dagger$, and hence $\calI_h^\dagger$, are independent of the information sets of action variables. That is, they only depend on the information structure of system variables.

Note that $\bbI_h^\dagger$ can contain system variables (observable or unobservable) as well as action variables. However, all action variables are assumed to be observable, and hence $\act(\bbI_h^\dagger) \subset \bbH_h$. In general, $\bbI_h^\dagger \not\subset \bbH_h$ since it may contain unobservable system variables.

The following proposition states that the rank of the observable dynamics of a sequential team is bounded by the cardinality of $\bbI_h^\dagger$. In particular, $i_h^\dagger \in \bbI_h^\dagger$ can be thought of as an \textit{information-structural state} in the sense that it describes a set of system variables, either observable or latent, which provide a sufficient statistic of the past at time $h$ for predicting future observations. Hence, the quantity $\aabs{\bbI_h^\dagger}$ admits an interpretation as the size of the information-structural effective state space at time $h$. This is a generalization of the standard notion of a latent state, as can be seen in the examples in~\Cref{sec:seq_teams_psr_rank_examples}.

\begin{proposition}[Rank of POSTs]\label{theorem:post_posg_rank}
    A partially-observable sequential team has a rank bounded by,
    \[r \leq \max_{h \in [H]} \bigl | \bbI_h^\dagger \bigr | .\]
\end{proposition}
\begin{proof}
    The proof is given in~\Cref{sec:appdx_seq_team_rank_proof}.
\end{proof}
% \begin{proof}
%     We have
%     \begin{equation*}
%         \begin{split}
%             \bra{\bm{D}_h}_{\tau_h, \omega_h} &=  \prob{\tau_h^o, \omega_h^o \given \mathrm{do}(\tau_h^a, \tau_h^a)} \\
%             &= \prob{\tau_h^o \given \mathrm{do}\paren{\tau_h^a}} \prob{\omega_h^o \given \tau_h^o;\,\mathrm{do}\paren{\tau_h^a, \omega_h^a}} \\
%             &\stepa{=} \prob{\tau_h^o \given \mathrm{do}\paren{\tau_h^a}} \sum_{\substack{x_k \in \bbX_k \\ k \in \calI_h^\dagger}} \prob{\set{x_k,\, k \in \calI_h^\dagger} \given \tau_{h}^o;\,\mathrm{do}\paren{\tau_h^a, \omega_h^a}} \prob{\omega_h^o \given \set{x_k,\, k \in \calI_h^\dagger}, \tau_h^o;\,\mathrm{do}\paren{\tau_h^a, \omega_h^a}} \\
%             &\stepb{=} \sum_{\substack{x_k \in \bbX_k \\ k \in \calI_h^\dagger}} \prob{\tau_h^o \given \mathrm{do}\paren{\tau_h^a}} \prob{\set{x_k,\, k \in \calI_h^\dagger} \given \tau_{h}^o;\,\mathrm{do}\paren{\tau_h^a}} \prob{\omega_h^o \given \set{x_k,\, k \in \calI_h^\dagger}, \tau_h^o;\,\mathrm{do}\paren{\tau_h^a, \omega_h^a}} \\
%             &\stepc{=} \sum_{\substack{x_k \in \bbX_k \\ k \in \calI_h^\dagger}} \prob{\tau_h^o \given \mathrm{do}\paren{\tau_h^a}} \prob{\set{x_k,\, k \in \calI_h^\dagger} \given \tau_{h}^o;\,\mathrm{do}\paren{\tau_h^a}} \prob{\omega_h^o \given \set{x_k,\, k \in \calI_h^\dagger};\,\mathrm{do}\paren{\omega_h^a}},
%         \end{split}
%     \end{equation*}
%     where step (a) is simply the law of total probability, step (b) is that $\{x_k, k \in \calI_h^\dagger\}$ is conditionally independent of $\mathrm{do}(\omega_h^a)$ (future actions) given $(\tau_{h}^o;\,\mathrm{do}(\tau_h^a))$ (the past), and step (c) is that $\omega_h^o$ is conditionally independent of $(\tau_h^o;\,\mathrm{do}(\tau_h^a))$ given $\{x_k,\, k \in \calI_h^\dagger\}$, by definition of $\calI_h^\dagger$ as the minimal set which $d$-separates $(X_{t(1)}, \ldots, X_{t(h)})$ from $(X_{t(h+1)}, \dots, X_{t(H)})$. Note that
%     \begin{equation*}
%         \prob{\set{x_k,\, k \in \calI_h^\dagger} \given \tau_{h}^o;\,\mathrm{do}\paren{\tau_h^a}} = \prob{\set{x_k,\, k \in \calI_h^\dagger \cap \calS} \given \tau_{h}^o;\,\mathrm{do}\paren{\tau_h^a}} \bm{1}\set{\paren{x_k,\, k \in \calI_h^\dagger \cap \calA} \ \text{matches} \ \tau_h^a},
%     \end{equation*}
%     since the action  components of $i_h^\dagger = (x_k, k \in \calI_h^\dagger)$ are contained in the history $\tau_h$.

%     Now define two matrices
%     \begin{equation*}
%         \begin{split}
%             \bm{D}_{h, 1} &\coloneqq \bra{\prob{\tau_h^o \given \mathrm{do}\paren{\tau_h^a}} \prob{\set{x_k,\, k \in \calI_h^\dagger} \given \tau_{h}^o;\,\mathrm{do}\paren{\tau_h^a}}}_{\tau_h, i_h^\dagger}, \quad \tau_h \in \bbH_h,\, i_h^\dagger \equiv \paren{x_k, \, k \in \calI_h^\dagger} \in \bbI_h^\dagger, \\%\set{(x_k)_{k \in \calI_h^\dagger} \in \prod_{k \in \calI_h^\dagger} \bbX_k} \\
%             \bm{D}_{h, 2} &\coloneqq \bra{\prob{\omega_h^o \given \set{x_k,\, k \in \calI_h^\dagger};\,\mathrm{do}\paren{\omega_h^a}}}_{i_h^\dagger, \omega_h}, \quad i_h^\dagger \equiv \paren{x_k, \, k \in \calI_h^\dagger} \in \bbI_h^\dagger,\, \omega_h \in \bbF_h.
%         \end{split}
%     \end{equation*}

%     We have that $\bm{D}_{h} = \bm{D}_{h,1} \bm{D}_{h,2}$, where both $\bm{D}_{h,1}$ and $\bm{D}_{h,2}$ have rank upper bounded by $\abs{\bbI_h^\dagger} = \prod_{s \in \calI_h^\dagger} \abs{\bbX_s}$. Hence, $\mathrm{rank}(\bm{D}_{h}) \leq \abs{\bbI_h^\dagger}$, and the result follows.
% \end{proof}

% The main idea of this result is that \textit{unobservable system variables can be used to obtain a lower-rank simplifications of the system dynamics}. A sequential team will have a smaller rank if its information structure is such that it contains (possibly unobserved) ``state-like'' variables which simplify the system dynamics and make the set $\bbI_h^\dagger$ smaller. In this sense, $\max_h \lvert \bbI_h^\dagger \rvert$ is a fundamental quantity which generalizes the notion of a ``state.''

% Given a particular information structure $\set{\calI_t, t \in \calN}$ for a sequential team, we can find $\calI_h^\dagger$ efficiently by constructing the corresponding DAG and applying $d$-separation algorithms for graphical models. There exists algorithms which run in linear time \parencite{tianFindingMinimalDseparators1998,zanderFindingMinimalDseparators2020}.

==> seq_teams_psr_rank_examples.tex <==
\section{Examples of Information Structures and their PSR rank}\label{sec:seq_teams_psr_rank_examples}

The procedure outlined in~\Cref{theorem:post_posg_rank} gives a way to obtain a low-rank decomposition of any partially-observable sequential team. Since POSTs and POSGs are general models which capture commonly studied models of sequential decision making like MDPs, POMDPs, POMGs, etc., this procedure recovers results about the rank of those models. Crucially, it also allows us to study additional sequential decision making problems with more complex information structures. In this section, we discuss how classical sequential decision-making models are special cases of POSTs/POSGs and how the rank of their system dynamics emerges from the graph-theoretic analysis of their information structure.

\textbf{Decentralized POMDPs and POMGs.} At each time $t$, the system variables of a decentralized POMDP (or POMG) consists of a latent state $s_t$, observations for each agent $o_t^1, \ldots, o_t^N$, and actions of each agent $a_t^1, \ldots, a_t^N$. The latent state transitions are Markovian and depend on the agents' joint action. The observations are sampled via a kernel conditional on the latent state. Each agent can use their own history of observations to choose an action. Thus, the information structure is given by,
\begin{equation*}
    \calI(s_t) = \set{s_{t-1}, a_{t-1}^1, \ldots, a_{t-1}^N},\, \calI(o_t^i) = \set{s_t},\, \calI(a_t^i) = \set{o_{1:t-1}^i, a_{1:t-1}^i}.
\end{equation*}
Here, the observable variables are $\calU = \set{o_{1:T}^i, a_{1:T}^i, i \in [N]}$\footnote{Here, since we don't explicitly write the index sets $\calS, \calO, \calA$ in the standard sequential teams formulation, we use the notation $\calI(x)$ to mean the information set $\calI_t$ where $x$ occurs at time $t$. In the case of Dec-POMDPs, since some events occur simultaneously, there is not a unique ordering of variables. For example, $(s_t, o_t^1, o_t^2)$ and $(s_t, o_t^2, o_t^1)$ are both valid orderings. When mapping such models onto the sequential teams framework, we may choose any ordering arbitrarily. Similarly, we slightly abuse notation when defining the set of observables $\calU$, where what we mean is the ``time indices'' of the variables in $\{\cdot\}$.}. By~\Cref{theorem:post_posg_rank}, we have $\calI^\dagger(o_t^i) = \calI^\dagger(a_t^i) = \set{s_t}, \, \forall t, i $, as shown in~\Cref{fig:decpomdp_I_dagger}. Thus, the PSR rank of a Dec-POMDP is bounded by $\abs{\bbS}$, where $\bbS$ is the state space. Note that in the case of models with a true latent state (e.g., POMDPs, Dec-POMDPs, and POMGs), the information-structural state coincides with the true latent state.

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[t]{0.6\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/dec_pomdp_min_separating_set.pdf}
        \caption{Decentralized POMDP/POMG information-structure.}\label{fig:decpomdp_I_dagger}
    \end{subfigure}

    \begin{subfigure}[t]{0.61\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mean_field_min_separating_set.pdf}
        \caption{``Mean-field'' information structure.}\label{fig:meanfield_I_dagger}
    \end{subfigure}
    \begin{subfigure}[t]{0.36\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/pt2pt_realtime_comm_w_feedback_min_separating_set.pdf}
        \caption{Point-to-point real-time communication with feedback information structure.}\label{fig:pt2pt_com_I_dagger}
    \end{subfigure}

    \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[width=\textwidth]{figures/2step_mem_min_separating_set.pdf}
        \caption{Limited-memory ($m=2$) information structures.}\label{fig:2step_mem_I_dagger}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\textwidth}
        \includegraphics[width=\textwidth]{figures/fully_connected_team_min_separating_set.pdf}
        \caption{Fully connected information structure.}\label{fig:fully_connected_I_dagger}
    \end{subfigure}
    \caption{DAG representation of various information structures. Solid edges indicate the edges in $\calE^\dagger$ and light edges indicate the information sets of action variables. Grey nodes represent unobservable variables, blue nodes represent past observable variables, green nodes represent future observable variables, and red nodes represent $\calI_t^\dagger$. To find $\calI_t^\dagger$, as per~\Cref{theorem:post_posg_rank}, we first remove the incoming edges into the action variables, then we find the minimal set among all past variables (both observable and unobservable) which $d$-separates the past observations from the future observations.}\label{fig:info_structs_dag}
\end{figure}

\textbf{Limited-memory information structures.} Consider a sequential decision making problem with variables $o_t, a_t, t \in [T]$ and an information structure with $m$-length memory. That is, observations can only depend directly on at most $m$ of the most recent observations and actions.
% Actions may still depend on the entire history of observations and past actions.
That is, the information structure is
\begin{equation*}
    \calI(o_t) = \set{o_{t-m:t-1}, a_{t-m:t-1}}, \calI(a_t) = \set{o_{1:t}, a_{1:t-1}}.
\end{equation*}

The observables are all observations and actions, $\calU = \set{o_{1:T}, a_{1:T}}$. By~\Cref{theorem:post_posg_rank} we have that $\calI^\dagger(o_t) = \set{o_{t-m:t-1}, a_{t-m:t-1}}$, as shown in~\Cref{fig:2step_mem_I_dagger}. Hence, the PSR rank of this sequential decision-making process is bounded by $\abs{\bbO}^{m} \abs{\bbA}^{m}$.

\textbf{Symmetric / ``Mean-field'' Information Structures.} Consider a sequential decision making problem with $N$ agents. Each agent has their own local state, $s_t^i \in \bbS_{\mathrm{local}}$. Similarly, at each time point, each agent takes an action $a_i^t \in \bbA_{\mathrm{loc}}$. The global state $s_t = (s_t^1, \ldots, s_t^N) \in \bbS_{\mathrm{loc}}^N =: \bbS$ is composed by of all agents' local states. Similarly, the joint action space is $\bbA \coloneqq \bbA_{\mathrm{loc}}^N$. Consider a symmetric information structure where the evolution of each agent's local state depends only on a symmetric aggregation of all agents' states and actions, rather than on the local state/action of any particular agent. That is, the identity of who is in what state or takes which action does not matter---only the distribution of states and actions. This is often referred to as a ``mean-field'' setting (in the limit). Here, the transition depends only on the distribution of local states and actions, defined as $s_t^{\mathrm{mf}} = \mathrm{dist}(s_t) \coloneq \frac{1}{N} \delta_{s_t^i}$, $a_t^{\mathrm{mf}} = \mathrm{dist}(a_t) \coloneq \frac{1}{N} \delta_{a_t^i}$, for $s_t \in \bbS, a_t \in \bbA$. Different agents can have different transition kernels for their local state.
% The observation variables are $\calO = \sset{s_{1:T}^i, i \in [N]}$ and the action variables are $\calA = \sset{a_{1:T}^i, i \in [N]}$.
Hence, by introducing $\mathrm{dist}(s_t), \mathrm{dist}(a_t)$ as auxiliary unobserved variables at each time $t$, we obtain the following information structure,
\begin{equation*}
    \calI(s_t^i) = \set{\mathrm{dist}(s_{t-1}), \mathrm{dist}(a_{t-1})}, \ \calI(a_t^i) = \set{s_t^i}
\end{equation*}
and an application of~\Cref{theorem:post_posg_rank} bounds the PSR rank by
\begin{equation*}
    \abs{\bbI^\dagger(s_t^i)} < \aabs{\bbS_{\mathrm{loc}}} \aabs{\bbA_{\mathrm{loc}}} \paren{\frac{N}{\aabs{\bbS_{\mathrm{loc}}} - 1} + 1}^{\aabs{\bbS_{\mathrm{loc}}} - 1} \paren{\frac{N}{\aabs{\bbA_{\mathrm{loc}}} - 1} + 1}^{\aabs{\bbA_{\mathrm{loc}}} - 1}.
\end{equation*}
This is compared to $\aabs{\bbS_{\mathrm{loc}}}^N \cdot \aabs{\bbA_{\mathrm{loc}}}^N$ (e.g., if we modeled this as an MDP with the state $s_t$), which is much larger when the number of agents is large. The information structure and $d$-separation decomposition are depicted in~\Cref{fig:meanfield_I_dagger}.

\textbf{Point-to-Point Real-Time Communication with Feedback.} Consider the following model of real-time communication with feedback. Let $x_t$ be the Markov source. At time $t$, the encoder receives the source $x_t \in \bbX$ and encodes sending a symbol $z_t \in \bbZ$. The symbol is sent through a memoryless noisy channel which outputs $y_t$ to the receiver. The decoder produces the estimate $\hat{x}_t$. The output of the noisy channel is also fed back to the encoder. The encoder and decoder have full memory of their observations and previous ``actions''. The observation variables are $\calO = \sset{x_{1:T},\, y_{1:T}}$ and the ``actions'' are $\calA = \sset{z_{1:T},\, \hat{x}_{1:T}}$. Hence, the information structure is given by the following,
\begin{equation*}
    \calI(x_t) = \set{x_{t-1}}, \ \calI(z_t) = \set{x_{1:t}, y_{1:t-1}, z_{1:t-1}}, \ \calI(y_t) = \set{z_{t}}, \ \calI(\hat{x}_t) = \set{y_{1:t}}.
\end{equation*}
By~\Cref{prop:seq_decmaking_exist_psr}, we have that,
\begin{equation*}
    \calI^\dagger(x_t) = \set{x_{t}}, \ \calI^\dagger(z_t) = \set{x_{t}}, \ \calI^\dagger(y_t) = \set{x_t, z_{t}}, \ \calI^\dagger(\hat{x}_t) = \set{x_{t}}.
\end{equation*}
Hence, the PSR rank is bounded by $\aabs{\bbX} \aabs{\bbZ}$. This is depicted in~\Cref{fig:pt2pt_com_I_dagger}.

\textbf{Fully-Connected Information Structures.} Consider a sequential decision making problem with variables $o_t, a_t, t \in [T]$ and a fully-connected information structure. That is, each observation directly depends on the entire history of observations and actions. Thus, the information structure is
\begin{equation*}
    \calI(o_t) = \set{o_{1:t-1}, a_{1:t-1}}, \calI(a_t) = \set{o_{1:t}, a_{1:t-1}}
\end{equation*}
The observables are all observations and actions, $\calU = \set{o_{1:T}, a_{1:T}}$. By~\Cref{theorem:post_posg_rank} we have that $\calI^\dagger(o_t) = \set{o_{1:t-1}, a_{1:t-1}}$, as shown in~\Cref{fig:fully_connected_I_dagger}. Hence, the PSR rank of this sequential decision-making process can be exponential in the time-horizon.

The examples above show that the tractability of a sequential decision-making problem (in terms of its rank) depends directly on its information structure. This gives an interpretation of why certain models, like POMDPs, are more tractable than those with arbitrary information structures. Previous work primarily considers particular problem classes with fixed and highly regular information structures. In this work we argue for the importance of explicitly modeling the information structure of a sequential decision-making problem.

% \textbf{Local Interaction on a time-varying network.} In the context of multi-agent systems, one way to interpret ``information structures'' is as a network of local interactions between agents in a (possibly time-varying) network. For example, consider again a sequential decision making problem with $N$ agents. Suppose that the interaction between agents is ``local'' in the sense that agent $j$'s local state and action at time $t$ only directly affects agent $i$'s local state transition at time $t+1$, if the two agents are connected in a (possibly time-varying) network, denoted by $\calN_t$. That is, we define the information structure as,
% \begin{equation*}
%     \calI(s_t^i) = \set{s_{t-1}^j, a_{t-1}^j : (j, i) \in \calN_t}.
% \end{equation*}

\begin{remark}[Necessity of generalized PSRs]\label{remark:necessity_gen_psr}
    The formalization of generalized PSRs in~\Cref{ssec:gen_psr} was necessary to enable the study of information structure as represented in partially-observable sequential teams. An alternative (naive) solution to construct PSR representations for models with non-alternating observations and actions (e.g., POST/POSG) is to aggregate consecutive observations and actions to force them to obey the standard formulation of PSRs. This approach results in a loss of ``resolution'' in the information structure of the underlying POST/POSG. That is, when you aggregate consecutive system variables, you also aggregate the DAG which represents the information structure, losing potentially important structure. In particular, in the worst case, such aggregation could result in an exponential increase in the rank of the system dynamics. The examples given above elucidate this. Consider for example the ``mean-field'' information structure. If we aggregated local states and actions into a combined global state and joint action, the rank would indeed be $\aabs{\bbS_{\mathrm{loc}}}^N \aabs{\bbA_{{\mathrm{loc}}}}^N$. By comparison, by considering each local state separately without aggregation, we are able to obtain a decomposition with a much smaller rank.
\end{remark}
